Using Synthetic Data and Deep Networks to Recognize Primitive Shapes for Object Grasping

A segmentation-based architecture is proposed to decompose objects into multiple primitive shapes from monocular depth input for robotic manipulation. The backbone deep network is trained on synthetic data with 6 classes of primitive shapes generated by a simulation engine. Each primitive shape is designed with parametrized grasp families, permitting the pipeline to identify multiple grasp candidates per shape primitive region. The grasps are priority ordered via proposed ranking algorithm, with the first feasible one chosen for execution. On task-free grasping of individual objects, the method achieves a 94% success rate. On task-oriented grasping, it achieves a 76% success rate. Overall, the method supports the hypothesis that shape primitives can support task-free and task-relevant grasp prediction.

==> related2.tex <==

\section{RELATED WORK}

%
% Traditional grasping method
%
Grasping is a fundamental problem in the robotics area. Earlier work relied on conventional analytical method which required a lot of prior knowledge of the target objects, such as geometry of the object, contact model and hand dynamics \cite{Murray_Li1994}\cite{bicchi2000robotic}. Although they could achieve promising results on the limited given objects, it is very hard for them to deal with other novel targets \cite{Tung_Kak_1996}\cite{Prattichizzo_Malvezzi_Gabiccini_Bicchi_2012}\cite{Rosales_Suarez_Gabiccini_Bicchi_2012}. 

%
% Deep Leaning grasping method
%
In the recent years, data-driven approaches have replaced the previous mainstream thanks to the success of deep learning \cite{Bohg_Morales_Asfour_Kragic_2014}\cite{caldera2018review}. 
%
% THREE WAYS OF METHODS: DETECTION, REINFORCEMENT LEARNING AND MODEL-BASED
%
Generally speaking, these methods could be concluded in three ways.
%
% DETECTION WAY
%
The first one tries to identify grasping as a detection problem with a structured grasping representation \cite{Watson_Hughes_Iida_2017}\cite{Park_Chun_2018}\cite{Chu_Xu_Vela_2018}. The idea is simple and straight forward. However, their predictions might be imprecise since the RGB or RGB-D training datasets like Cornell \cite{lenz2015deep} and Jacquard \cite{depierre2018jacquard} are easily affected by the light, color or other environment factors. DexNet \cite{mahler2017dex} proposed by Mahler \textit{et al.} could achieve  superior performance thanks to the large volume dataset, but it still requires high quality depth input.
%
% REINFORCEMENT LEARNING
%
Another group of researchers focuses on the emerging reinforcement learning tactic. This intuitive method based on the trial-and-error idea presents a good performance without any data annotation cost \cite{levine2018learning}\cite{zeng2018learning}\cite{mahler2019learning}. Unfortunately, it requires hundreds of thousand of experiments to train the policy, which is extremely time-consuming. 
%
% MODEL-BASED
%
The rest people mainly address grasping problem with model-based methods. 
%
% BASIC IDEA OF PRIMITIVE SHAPES
%
When confronted with a difficult grasping problem, people unconsciously tend to simplify the task by decomposing the complicated shape into several primitive shapes which they are more familiar with \cite{miller2003automatic}. Inspired by this fact, primitive shapes is developed as an intuitive approach to generalize a variety of objects. 

% INTRODUCE SOME PREVIOUS WORK ABOUT PRIMITIVE SHAPES
% 
% SOME WORKS INTRODUCED THE IDEA OF DECOMPOSING COMPLICATED OBJECTS
%
A variety of methods have been proposed based on this idea. Miller \textit{et al.} \cite{miller2003automatic} made the use of primitive shapes for better grasping configuration selection. Similarly, Yamanobe \textit{et al.} \cite{yamanobe2010grasp}\cite{shiraki2014modeling} showed the advantage of  decomposing complicated objects with several primitive shapes. However, the methods mentioned above just proposed the concept of decomposition but actually annotated the target object model manually for testing. 
%
% SOME WORKS FOCUSED ON DECOMPOSING OBJECTS AUTOMATICALLY
%
With the advent of advanced segmentation algorithms, researchers started to focus on automatically decomposing the objects.
%
Goldfeder \textit{et al.} \cite{Goldfeder_Allen_Lackner_Pelossof_2007} decomposed the 3D model into a superquadric decomposition tree with the help
of \cite{Laurent2003}. However, this two-stage segmentation approach based on split and merge procedures is sensitive to the missing data of the point cloud , which is a common case in the monocular vision system. 
%
Alternatively, Huebner \textit{et al.} \cite{huebner2008selection} introduced the idea of box-based shapes into the grasping problem instead of designing different types of primitive shapes, but their decomposition algorithm \cite{huebner2008minimum} is too coarse to abstract the target object with high accuracy. 
%
% REPRESENT EVERY OBJECT WITH A SINGLE PRIMITIVE SHAPE
%
On the other hand, some methods simplify the problem by representing every object with a single primitive shape. 
%
For example, Jain \textit{et al.} \cite{jain2016grasp} employed RANSAC \cite{fischler1981random} algorithm to generate model hypotheses and performed Euclidean clustering to segment the target object from the point cloud input.

% DIFFERENCES BETWEEN OUR WORK AND SOME HIGHLY RELATED ONES
%
Different from all these analytical methods mentioned above, our work builds up a dataset of primitive shapes combinations inspired by Tobin \textit{et al.}'s methodology \cite{tobin2017domain} of data generation, which could cover a large scope of objects. Furthermore, instead of training a simple detection network \cite{tobin2017domain}, the state-of-the-art instance segmentation approach Mask R-CNN \cite{he2017mask} is employed as our backbone network to segment a 2D image into different parts of primitive shapes. In this way, our algorithm is able to implement task-oriented grasping \cite{fang2018learning}. Specially, we take a monocular depth image as the input to avoid the disturbance of texture or light information \cite{Yang2018}.
>>>>>>> ce5c9860d66f61e1183a26a4c368278871ec1b4a

